Inverting and Understanding Object Detectors

As a core problem in computer vision, the performance of object detection has improved drastically in the past few years. Despite their impressive performance, object detectors suffer from a lack of interpretability. Visualization techniques have been developed and widely applied to introspect the decisions made by other kinds of deep learning models; however, visualizing object detectors has been underexplored. In this paper, we propose using inversion as a primary tool to understand modern object detectors and develop an optimization-based approach to layout inversion, allowing us to generate synthetic images recognized by trained detectors as containing a desired configuration of objects. We reveal intriguing properties of detectors by applying our layout inversion technique to a variety of modern object detectors, and further investigate them via validation experiments: they rely on qualitatively different features for classification and regression; they learn canonical motifs of commonly co-occurring objects; they use diff erent visual cues to recognize objects of varying sizes. We hope our insights can help practitioners improve object detectors.

==> figures/surrounding_anchor.tex <==
\begin{figure}
\centering
    \begin{subfigure}
        \centering
        \includegraphics[width=.23\textwidth]{./image/Surrounding/png/person_bar_3_0.png}
        \includegraphics[width=0.23\textwidth]{./image/Surrounding/png/person_bar_3_2.png}
    \end{subfigure}
    \vspace{-5mm}
    \caption{We display the emerging surrounding contexts while visualizing individual person at 3-rd scale
    with different anchor ratio: 1:2 anchor for left and 2:1 anchor for right.}
    \label{fig:sur_anchor}
    \vspace{-5mm}
\end{figure}

==> image/figure4_loss_abalation/loss_abalation.tex <==
\begin{figure*}
\centering
\begin{tabular}{@{}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{}}
\small \text{layout} &
\small \text{All loss} & 
\small \text{layout} &
\small \text{All loss} & 
\small \text{layout} &
\small \text{All loss} \\


\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072_full.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}\\

\small \text{Cls} &
\small \text{Reg-Mask} & 
\small \text{Cls} &
\small \text{Reg-Mask} & 
\small \text{Cls} &
\small \text{Reg-Mask} \\

\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072_cls.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072_reg_mask.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}\\

\small \text{Reg} &
\small \text{Cls-Mask} & 
\small \text{Reg} &
\small \text{Cls-Mask} & 
\small \text{Reg} &
\small \text{Cls-Mask} \\

\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072_reg.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072_cls_mask.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}\\

\small \text{Mask} &
\small \text{Cls-Reg} & 
\small \text{Mask} &
\small \text{Cls-Reg} & 
\small \text{Mask} &
\small \text{Cls-Reg} \\

\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072_mask.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure4_loss_abalation/jpg/000000055072_cls_reg.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}&
\includegraphics[width=0.165\textwidth]{./image/000000439715.jpg}\\


\end{tabular}
\caption{Vis Ablation experiment}
\label{Visual_Interpolation}
\end{figure*}


==> image/figure6_neuron_category/neuron_category.tex <==
\begin{figure}
\centering
\begin{tabular}{@{}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{}}
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_0_scale3_anchor_2_1_retina.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_77_scale3_anchor_2_2_retina.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_2_scale3_anchor_0_1_retina.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_5_scale3_anchor_1_0_retina.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_15_scale3_anchor_0_1_retina.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_1_scale3_anchor_0_0_retina.jpg}\\
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_0_scale3_anchor_2_1_faster.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/cateogry_77_scale3_anchor_2_2_faster.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_2_scale3_anchor_0_2_faster.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/cateogry_5_scale3_anchor_1_1_faster.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/cateogry_15_scale3_anchor_0_1_faster.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure6_neuron_category/jpg/category_1_scale3_anchor_0_1_faster.jpg}\\
\small \text{Person} &
\small \text{Teddy bear}&
\small \text{Car}&
\small \text{Bus}&
\small \text{Cat}&
\small \text{Bicycle}
\\
\end{tabular}
\caption{Class-Specific Visualization for RetinaNet.}
\label{class-specific}
\end{figure}

==> image/figure7_neuron_scale/neuron_scale.tex <==
\begin{figure*}
\centering
\begin{tabular}{@{}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{\hspace{0.7mm}}c@{}}
\tiny \text{RetinaNet-F-R50} &
\tiny \text{RetinaNet-F-R101} &
\tiny \text{Faster-RCNN-F-R50} &
\tiny \text{Faster-RCNN-C-R50}&
\tiny \text{Faster-RCNN-F-R101}&
\tiny \text{Faster-RCNN-C-R101}\\

\rotatebox{90}{Scale 1}
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_50_category0_scale0_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_101_category0_scale0_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_F_category0_scale0_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_C_category0_scale0_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_F_category0_scale0_anchor_2_2.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_C_category0_scale0_anchor_2_0.jpg}\\

\rotatebox{90}{Scale 2}
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_50_category0_scale1_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_101_category0_scale1_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_F_category0_scale1_anchor_2_2.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_C_category0_scale1_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_F_category0_scale1_anchor_2_2.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_C_category0_scale1_anchor_2_0.jpg}\\

\rotatebox{90}{Scale 3}
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_50_category0_scale2_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_101_category0_scale2_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_F_category0_scale2_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_C_category0_scale2_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_F_category0_scale2_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_C_category0_scale2_anchor_2_0.jpg}\\

\rotatebox{90}{Scale 4}
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_50_category0_scale3_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_101_category0_scale3_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_F_category0_scale3_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_C_category0_scale3_anchor2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_F_category0_scale3_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_C_category0_scale3_anchor_2_1.jpg}\\

\rotatebox{90}{Scale 5}
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_50_category0_scale4_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/retina_101_category0_scale4_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_F_category0_scale4_anchor_2_0.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_50_C_category0_scale4_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_F_category0_scale4_anchor_2_1.jpg}&
\includegraphics[width=0.165\textwidth]{./image/figure7_neuron_scale/jpg/faster_101_C_category0_scale4_anchor_2_2.jpg}\\
\end{tabular}
\caption{Neuron Visualization for different RPN scale.}
\label{Visual_RPN_Scale}
\end{figure*}

